SpecInfer: Accelerating Generative Large Language Model Serving with Tree-based Speculative Inference and Verification

This paper introduces SpecInfer, a system that accelerates generative large language model (LLM) serving with tree-based speculative inference and verification. The key idea behind SpecInfer is leveraging small speculative models to predict the LLM's outputs; the predictions are organized as a token tree, whose nodes each represent a candidate token sequence. The correctness of all candidate token sequences represented by a token tree is verified against the LLM in parallel using a novel tree-based parallel decoding mechanism. SpecInfer uses an LLM as a token tree verifier instead of an incremental decoder, which significantly reduces the end-to-end latency and computational requirement for serving generative LLMs while provably preserving model quality. Our evaluation shows that SpecInfer outperforms existing LLM serving systems by 1.5-2.8x for distributed LLM inference and by 2.6-3.5x for offloading-based LLM inference, while preserving the same generative performance. SpecInfer is publicly available at https://github.com/flexflow/FlexFlow/

==> background.tex <==
\section{Background}
\label{sec:background}

==> discussion.tex <==
\section{Discussion}


==> table/CBT-LLaMA.tex <==
\if 0
\begin{table}
\begin{center}
% \caption{Average number of tokens verified by \Sys in a decoding step.  We used \llama-7B as the LLM and used different numbers of collectively boost-tuned SSMs, all of which were derived from \llama-160M. The speculation length is 16 for all SSMs.}
\caption{\textcolor{blue}{Llama 68M naive sample (this caption and table label need to be modified).}}
\footnotesize
\label{tab:cbt-llama}
\begin{tabular}{ccccccc}
\toprule
\# Tree Width  &base    & 1 & 2 & 3 & 4 & 5 \\ \midrule
Alpaca     &1.34     & 1.41     & 1.68    & 1.76     & 1.82     & \textbf{1.87}     \\
CP         &1.32     & 1.37     & 1.57    & 1.63     & 1.71     & \textbf{1.80}     \\
WebQA      &1.34     & 1.38     & 1.58    & 1.65     & 1.69     & \textbf{1.73}     \\
CIP        &1.33     & 1.39     & 1.60    & 1.67     & 1.74     & \textbf{1.79}     \\
PIQA       &1.36     & 1.41     & 1.58    & 1.65     & 1.69     & \textbf{1.73}         \\ \midrule
Avg        &1.34     & 1.39     & 1.60    & 1.67     & 1.73     & \textbf{1.79}      \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\fi 


\begin{table}
\begin{center}
\caption{Average number of tokens verified by \sys in a decoding step.  We used \llama-7B as the LLM and used different tree widths for constructing a token tree. The speculation length is 8 for all experiments.}
%\caption{\textcolor{blue}{Llama 68M improved sample (this caption and table label need to be modified).}
%\footnotesize
\label{tab:cbt-llama}
\begin{tabular}{ccccccc}
\toprule
\# Tree Width  & base   & 1 & 2 & 3 & 4 & 5 \\ \midrule
Alpaca     &1.71     & 1.79     & 2.11    & 2.26     & 2.32     & \textbf{2.38}     \\
CP         &1.63     & 1.69     & 1.99    & 2.15     & 2.23     & \textbf{2.28}     \\
WebQA      &1.57     & 1.64     & 1.93    & 2.08     & 2.15     & \textbf{2.21}     \\
CIP        &1.68     & 1.72     & 2.05    & 2.19     & 2.28     & \textbf{2.29}     \\
PIQA       &1.62     & 1.67     & 1.93    & 2.08     & 2.15     & \textbf{2.21}         \\ \midrule
Avg        &1.64     & 1.70     & 2.00    & 2.15     & 2.23     & \textbf{2.28}      \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
% \caption{Average number of tokens verified by \Sys in a decoding step.  We used \llama-7B as the LLM and used different numbers of collectively boost-tuned SSMs, all of which were derived from \llama-160M. The speculation length is 16 for all SSMs.}
\caption{\textcolor{blue}{Llama 68M greedy decoding (this caption and table label need to be modified).}}
\footnotesize
\label{tab:cbt-llama}
\begin{tabular}{l|cccccc}
\toprule
        \# Tree Width  &base   & 1 & 2 & 3 & 4 & 5 \\ \midrule
Alpaca     &2.81     & 2.95     & 3.07    & 3.21     & 3.33     & \textbf{3.43}     \\
CP         &2.42     & 2.58     & 3.24    & 3.46     & 3.59     & \textbf{3.69}     \\
WebQA      &2.10     & 2.27     & 2.69    & 2.86     & 2.98     & \textbf{3.07}     \\ 
CIP        &2.63     & 2.73     & 3.40    & 3.62     & 3.79     & \textbf{3.91}     \\
PIQA       &2.04     & 2.18     & 2.80    & 2.97     & 3.10     & \textbf{3.21}     \\   \midrule
Avg        &2.40     & 2.54     & 3.04    & 3.22     & 3.36     & \textbf{3.46}      \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

\if 0
\begin{table}
\begin{center}
% \caption{Average number of tokens verified by \Sys in a decoding step.  We used \llama-7B as the LLM and used different numbers of collectively boost-tuned SSMs, all of which were derived from \llama-160M. The speculation length is 16 for all SSMs.}
\caption{\textcolor{blue}{Llama 68M greedy decoding top-k accept rate (this caption and table label need to be modified).}}
\footnotesize
\label{tab:cbt-llama}
\begin{tabular}{cccccc}
\toprule
           Top-k     & 1 & 2 & 3 & 4 & 5 \\ \midrule
Alpaca     &0.68          & 0.77    & 0.81     & 0.84     & \textbf{0.85}     \\
CP         &0.69          & 0.79    & 0.83     & 0.86     & \textbf{0.87}     \\
WebQA      &0.62          & 0.72    & 0.77     & 0.80     & \textbf{0.82}     \\ 
CIP        &0.70          & 0.81    & 0.85     & 0.88     & \textbf{0.89}     \\
PIQA       &0.63          & 0.75    & 0.79     & 0.83     & \textbf{0.85}     \\   \midrule
Avg        &0.66          & 0.77    & 0.81     & 0.84     & \textbf{0.86}      \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
% \caption{Average number of tokens verified by \Sys in a decoding step.  We used \llama-7B as the LLM and used different numbers of collectively boost-tuned SSMs, all of which were derived from \llama-160M. The speculation length is 16 for all SSMs.}
\caption{\textcolor{blue}{Llama 68M improved sampling top-k accept rate (this caption and table label need to be modified).}}
\footnotesize
\label{tab:cbt-llama}
\begin{tabular}{cccccc}
\toprule
           Top-k     & 1 & 2 & 3 & 4 & 5 \\ \midrule
Alpaca     &0.54          & 0.81    & 0.91     & 0.95     & \textbf{0.97}     \\
CP         &0.56          & 0.82    & 0.92     & 0.95     & \textbf{0.97}     \\
WebQA      &0.52          & 0.80    & 0.90     & 0.94     & \textbf{0.96}     \\ 
CIP        &0.57          & 0.84    & 0.92     & 0.95     & \textbf{0.97}     \\
PIQA       &0.55          & 0.82    & 0.91     & 0.95     & \textbf{0.97}     \\   \midrule
Avg        &0.55          & 0.82    & 0.91     & 0.95     & \textbf{0.97}      \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\fi

==> table/CBT-OPT.tex <==
\begin{table}
\caption{Average number of tokens verified by \Sys in a decoding step. We used OPT-13B as the LLM and used different numbers of collectively boost-tuned SSMs, all of which were derived from OPT-125M. The speculation length is 16 for all SSMs.}
\label{tab:cbt-opt}
\begin{center}
\footnotesize
\begin{tabular}{cccccc}
\toprule
               \# SSMs             & 1 & 2 & 3 & 4 & 5 \\ \midrule
CIP & 3.00     & 3.39     & 3.52     & 3.58     & \textbf{3.74}     \\
CP           & 2.95     & 3.35     & 3.49     & 3.52     & \textbf{3.68}     \\
WebQA                      & 2.51     & 2.92     & 3.04     & 3.09     & \textbf{3.20}     \\
Alpaca               & 3.33     & 3.89     & 4.06     & 4.17     & \textbf{4.35}     \\
PIQA                        & 2.75     & 3.14     & 3.26     & 3.31     & \textbf{3.43}     \\ \midrule
Avg                         & 2.91     & 3.34     & 3.47     & 3.53     & \textbf{3.68}     \\ \bottomrule
\end{tabular}
\end{center}
\end{table}

==> table/LSS-OPT.tex <==
% \if 0
% \begin{table}[H]
% \caption{\XM{TODO: add a caption}}
% \label{tab:lss-opt}
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
%         & \multicolumn{2}{c}{CIP} & \multicolumn{2}{c}{CP} & \multicolumn{2}{c}{WebQA} & \multicolumn{2}{c}{Alpaca} & \multicolumn{2}{c}{PIQA} \\ \cline{2-11} 
%         & w/ oracle  & w/o oracle & w/ oracle & w/o oracle & w/ oracle   & w/o oracle  & w/ oracle   & w/o oracle   & w/ oracle  & w/o oracle  \\ \hline
% LLM Run & 8812       & 8449       & 3625      & 3462       & 12624       & 12080       & 11123       & 10684        & 12625      & 11560       \\
% SSM Run & 56401      & 135184     & 23172     & 55392      & 74953       & 193280      & 72863       & 170944       & 74548      & 184960      \\ \hline
% \end{tabular}
% \end{center}

% \end{table}

\begin{table}
\caption{The number of LLM runs and SSM runs with or without the presence of the matching length predictor. When there is no predictor, we use a fixed speculation length of 16 for all the SSMs in this experiment. LLM: OPT-13B, SSMs: OPT-125M}
\label{tab:lss-opt}
\begin{center}
\begin{tabular}{ccccc}
\toprule
       & \multicolumn{2}{c}{LLM run} & \multicolumn{2}{c}{SSM run} \\ \cmidrule{2-5} 
       & w/ predictor    & w/o predictor   & w/ predictor    & w/o predictor   \\ \midrule
CIP    & 8812         & 8449         & 56401        & 135184       \\
CP     & 3625         & 3462         & 23172        & 55392        \\
WebQA  & 12624        & 12080        & 74953        & 193280       \\
 Alpaca & 11123        & 10684        & 72863        & 170944       \\
PIQA   & 12625        & 11560        & 74548        & 184960       \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
% \fi 
